BaPu: Efficient and Practical Bunching of Access Point Uplinks

Today's increasing demand for wirelessly uploading a large volume of User Generated Content (UGC) is still significantly limited by the throttled backhaul of residential broadband (typically between 1 and 3Mbps). We propose BaPu, a carefully designed system with implementation for bunching WiFi access points' backhaul to achieve a high aggregated throughput. BaPu is inspired by a decade of networking design principles and techniques to enable efficient TCP over wireless links and multipath. BaPu aims to achieve two major goals:1) requires no client modification for easy incremental adoption; 2) supports not only UDP, but also TCP traffic to greatly extend its applicability to a broad class of popular applications such as HD streaming or large file transfer. We prototyped BaPu with commodity hardware. Our extensive experiments shows that despite TCP's sensitivity to typical channel factors such as high wireless packet loss, out-of-order packets arrivals due to multipath, heterogeneous backhaul capacity, and dynamic delays, BaPu achieves a backhaul aggregation up to 95% of the theoretical maximum throughput for UDP and 88% for TCP. We also empirically estimate the potential idle bandwidth that can be harnessed from residential broadband.

==> bapu_pro.tex <==
\section{Bapu}
\label{sec:bapu-pro}

Inspired by our analysis in section \ref{sec:bapubasic-tcp}, we propose BaPu-Pro to address
the TCP challenges. BaPu-Pro shares the same architecture as BaPu-Basic, and employs
a mechanism called \emph{Proactive-ACK} to mitigate the out-of-order TCP sequence issue. 
BaPu-Pro maintains a healthy CWND growth at the sender side, and therefore achieves high throughput.

\subsection{Proactive-ACK}

The protocol flow of BaPu-Pro is depicted in Figure \ref{fig:bapu-pro-flow}. At a high level, 
BaPu-Pro works as follow,
\begin{enumerate}
\item BaPu-APs send packet reception report to BaPu-Gateway.  The only difference from BaPu-Basic at this step is
that each report includes the TCP sequence number of the reported packet. 
\item BaPu-Gateway maintains a lookup table to record all the the reported TCP sequence.   
\item On receiving a new TCP sequence, BaPu-Gateway scans the table to find out if a continuous sequence has been reported. If so, BaPu-Gateway generates a series of spoofed TCP ACKs and sends them to the sender.  The intuition is that all the reported sequence numbers are currently buffered at some BaPu-AP, and due to the reliability of the TCP tunnel between the BaPu-AP and the BaPu-Gateway, will be reliably forwarded to the BaPu-Gateway ultimately.  Therefore, as long as BaPu-Gateway identifies a continuous range of reported TCP sequence, it is safe to send acknowledgement back to the sender.  Such spoofed ACKs may happen even before the real TCP segments are forwarded to the BaPu-Gateway. In this way, the TCP sequence window at the sender side can keep sliding which prevents the ACK timeout from happening.  
\item If the report for next expected TCP sequence is not received within certain time window, it is likely that this sequence is lost on all BaPu-APs. In this case, BaPu-Gateway sends a spoofed DUPACK back to the sender. Such operation mimics the TCP Fast Retransmission mechanism for fast recovery from potential packet loss.
%\item As BaPu-Gateway receives the IP packets from the tunnel, it starts forwarding the IP packets to the destination only when the next expected TCP sequence is ready.  Otherwise, the out-of-order TCP segments will be buffered at BaPu-Gateway until the expected sequence arrives.  Such strategy ensures that the destination always receives in order TCP segments.  Its advantage is that the destination always generates normal TCP ACK, rather than DUPACK or selective ACK. This simplifies the logic to maintain the TCP semantic.
\item As BaPu-Gateway forwards the received TCP segment to the destination, the destination will send real TCP ACKs to the sender.  Since BaPu-Gateway resides along the path between the sender and the destination, BaPu-Gateway captures the pure TCP ACKs and discards them.  We discard the real TCP ACKs because we have already sent a spoofed ACK to the sender a while ago. 
\item The destination may send TCP data segment to the sender.  For those packets, BaPu-Gateway just let them go along the default network path. 
\end{enumerate}

\begin{figure}
\centering
\includegraphics[width=0.9\columnwidth]{figures/bapu-pro-flow-compact}
\vspace{-0.1in}
\caption{BaPu-Pro Protocol Traffic Flow}
\label{fig:bapu-pro-flow}
\end{figure}

TCP is two way communication. Both ends may send TCP data packets to each other. Thus, the sequence window at both ends must be properly synchronized.  Asides from the sequence number, other TCP header fields are also important. For example, the advertised receiver window size is important for flow control between sender and receiver. To honour the TCP header fields generated by the receiver, BaPu-Gateway monitors the real TCP ACKs generated by the destination.  BaPu-Gateway extracts the TCP header and use those values to prepare the spoofed ACKs. While the Proactive-ACK mechanism breaks the end to end semantic of TCP, BaPu can be limited to operate on HTTP upload (POST) traffic which has an explicit application layer acknowledgment mechanism (i.e., HTTP 200 OK).

\ignore{
\paragraph{Implementation}
Based on the implementation of BaPu-Basic described in section~\ref{sec:implement}, we integrate 
the Proactive-ACK mechanism at BaPu-Gateway. 
BaPu-Gateway uses \emph{raw socket} to spoof the TCP ACKs. We also install proper iptables rules at BaPu-Gateway 
and use \emph{iptables-queue} to capture the returning TCP traffic from the destination to the sender.
BaPu-AP logic remains unmodified. }



==> design.tex <==
\section{BaPu}
\label{sec:design}
%% briefly emphasize BaPu's function
BaPu is a suite of software solutions running on the home WiFi APs 
and gateway servers.  BaPu consists of the two major components, 

\begin{itemize}
\item \textit{BaPu-AP}: In BaPu, each home WiFi AP is configured as both AP 
mode and monitor mode. In an upload session, the sender carries out unicast to 
its own home AP via a high bandwidth wireless link.   The proximate BaPu-APs
overhears the communication in monitor mode. 
This group of BaPu-APs, including both home-AP and monitor-APs, 
communicate with the far end BaPu-Gateway to determine which AP forwards which 
IP packet.  
\ignore{The scheduled IP packets are forwarded from the BaPu-AP to the 
BaPu-Gateway through a TCP tunnel connection.  In this way, the \textbf{``fat"} 
wireless data flow is forwarded to the destination utilizing multiple APs' 
backhaul uplinks. }

\item \textit{BaPu-Gateway}: To make traffic multiplexing transparent to 
both sender and destination, we design BaPu-Gateway, 
which resides on the network path between the BaPu-APs and the destination. 
BaPu-Gateway is mainly responsible for scheduling and load balancing on
BaPu-APs, and forwarding the traffic to the destination. 
BaPu-Gateway may be deployed in the following 3 scenarios: 
1) The destination is an end device in a WLAN. The BaPu-Gateway runs on the WiFi 
AP of the same WLAN; 2) The destination is a server where the data is uploaded 
to.  The BaPu-Gateway is a gateway server running in front of it; 3) The 
BaPu-Gateway and the destination reside on the same physical machine.  
The destination is a service process which receives the uploaded data, while 
the BaPu-Gateway is a process intercepting on the data propagation path to 
the destination.
\end{itemize}

%% bapu's relies on three major mechanisms: tunnel forwarding, scheduling and load balancer 
The main idea of our BaPu system is inspired by the work from Jakubczak et al. 
\cite{link-alike}. Our preliminary experiments show that we can achieve high 
aggregated throughput with efficiency over 95\% for UDP. However,
 the basic design performs poorly for TCP due to some of TCP's 
 inherent nature. Therefore, we call this solution ``BaPu-Basic".  In the contrast, 
 we propose a novel mechanism \emph{Proactive-ACK} to improve the TCP performance,
 which we call ``BaPu-Pro".  In the following 
 section, we first present BaPu-Basic mechanisms in detail and our preliminary evaluation 
 of BaPu-Basic. Then we present
 an analysis on why BaPu-Basic is not adequate for TCP.

\subsection{Client Transparent Tunnel Forwarding}

Figure \ref{fig:bapu-basic-flow} describes the BaPu-Basic protocol traffic flow.
As the sender device transfers data to its home-AP $H$, the proximate monitor-AP(s), 
$M_1$, overhears the wireless communication.  BaPu-AP identifies a 
transport session based on the following tuple, 

$<BSSID, protocol, src IP, dst IP, src Port, dst Port>$\\
Here $protocol$ indicates whether it is a TCP or UDP session. The latter five items 
are the typical tuple to identify a transport layer session. However, in neighboring 
WLANs, the clients may have conflicting IP addresses. To resolve such conflict, we 
use $BSSID$ in the 802.11 header to identify which WLAN this session belongs to. 

Once BaPu-AP identifies a new session, it establishes a TCP connection to the $dst IP$, 
which is the IP address of the BaPu-Gateway $G$. BaPu-AP registers itself at the 
BaPu-Gateway for the newly identified session. On registration, BaPu-Gateway assigns 
each BaPu-AP an AP ID.  Later on, the tunnelled IP packets and exchanged control 
information is all carried through this TCP tunnel.
At $H$, instead of directly forwarding the sender's packets to the Internet, 
it stores the packets in a session buffer.  Session buffer is a memory space allocated 
for each BaPu session, and will be released when the session ends.  
Similarly, the monitor-APs all maintain a session buffer to store the overheard packets. 
In order to harness the idle bandwidth of multiple APs, BaPu-APs and BaPu-Gateway 
coordinate to determine how to split the traffic load.  Therefore, the bandwidth 
aggregation is transformed to the problem of how to schedule the packets
among BaPu-APs.  BaPu adopts a centralized scheduling mechanism at BaPu-Gateway. 
For example, $H$ and $M_1$ both 
receive packet $p$, and each sends packet reception report to $G$. Based on our 
scheduling method, $G$ schedules $M_1$ to forward IP packet $p$.  We will explain our scheduling mechanism in next section.   
$G$ informs all BaPu-APs of this scheduling decision.  Upon receiving the schedules, 
$H$ releases packet  $p$ from its session buffer.  $M_1$ carries out the following two operations,
\begin{itemize}
\item \textbf{NAT}: The sender is behind a home-AP, which is generally also a NAT. In this case, the packet overheard by $M_1$ has the private IP address.  $M_1$ first translates the private IP/port pair to the public pair. The home-AP and BaPu-Gateway can communicate to obtain the NAT mapping record for this session. The monitor-AP can retrieve the NAT mapping record when it establishes the tunnel connection with BaPu-Gateway. Please note that the NAT operation is not mandatory at AP side. We can shift the NAT operation to the BaPu-Gateway.  
\item \textbf{Encapsulation}: $M_1$ encapsulates the NAT'ed IP packet in our BaPu protocol message and sends it to the BaPu-Gateway. 
\end{itemize}

When BaPu-Gateway receives the tunnelled packets, it simply inject the packets to the network with raw socket.  The packet is then finally delivered to the destination. 

A few points are worth noting,

\begin{enumerate}
\item In BaPu, we assume that the downlink capacity has no limit. Thus, all the downlink traffic from the destination to the sender still goes along the default path.  Since the sender may reside behind multiple tiers of NAT boxes, we must ensure that the NAT mapping for this session is properly installed on all NAT boxes along the path between sender and destination, so that the returning traffic can traverse the NAT boxes properly.  Therefore, the first few packets in a session must go along the default path.  This generally means the first packet in UDP session or the 3-way handshake traffic in TCP session.  

\item Compared with UDP, TCP obviously has higher overhead.  However, the choice of TCP tunnels is partially motivated by TCP-friendliness. We want to aggregate the idle bandwidth without overloading the ISP's networks. Besides, since TCP tunnel can provide a reliable channel,  it also helps keep a simple logic for the control and data communication between BaPu-AP and BaPu-Gateway.

\item In theory, the monitor-APs can send NAT'ed IP packet with raw socket, instead of forwarding it through the tunnel. This seems more straightforward.  However, it is inapplicable for two reasons: 1) many ISPs block the spoofed IP packet; 2) raw TCP socket is not reliable.
\end{enumerate}

\begin{figure}
\centering
\includegraphics[width=0.9\columnwidth]{figures/bapu-basic-flow-compact}
\vspace{-0.1in}
\caption{BaPu-Basic Protocol Traffic Flow}
\label{fig:bapu-basic-flow}
\end{figure}

\subsection{Scheduling}
\label{sec:schedule}
%% Why scheduling is important 
%% Link-alike discussed on 3 possible scheduling design
As mentioned above, the bandwidth aggregation is transformed to the problem of how to schedule the IP packet forwarding among BaPu-APs to make the best utilization of the limited uplink capacity.  As we design the scheduler, we explored 3 mechanisms, \textbf{module scheduler}, \textbf{module+redundancy} and \textbf{centralized scheduler}. 

In \textbf{module scheduler}, each BaPu-AP computes a hash value for IP ID.  The hash function is defined to have low enough collision probability.  If the IP ID moduled by AP ID is 0, the BaPu-AP forwards this packet. Otherwise, BaPu-AP discards it. 
The big advantage of module scheduler is zero coordination overhead.  However, the major downside of module scheduler is its unreliability.  Due to the WiFi packet loss, the BaPu-AP, which should forward certain packet, may not receive this packet. In this case, this packet is for sure lost, which results in throughput degradation. Such packet loss can lead to even worse throughput in TCP. 

In order to mitigate the packet loss in module scheduler, we attempt to introduce some redundancy.  We examined one simple strategy, \textbf{P-based redundancy}.  In P-based redundancy, other than the packets selected by the module function, each BaPu-AP also forwards the received packets with some pre-determined random probability P.  Even though such redundancy in packet forwarding can mitigate the packet loss.  However, it places a bottleneck on the maximum achievable throughput because each BaPu-AP forwards packets in probability P, which results in a waste of bandwidth.  

In our design, we adopt a \textbf{centralized scheduler} at BaPu-Gateway.  BaPu-AP sends a packet reception report to BaPu-Gateway for each received packet.  With the complete knowledge of packet reception at all BaPu-APs, BaPu-Gateway determines which AP should forward which packet.  Also, with this centralized design, it is easy to employ extra logic to further optimize the scheduling strategy, such as the load balancing method which we will present in next section. 
At the centralized scheduler, we choose First-Come First-Served (FCFS) strategy to select the BaPu AP for forwarding the packet. The intuition of FCFS is that, among APs who have enough bandwidth to transmit the data, the AP which reports first should forward the packet in order to deliver the reported packet as soon as possible. Our design matches the approach taken in Link-alike \cite{link-alike}.  However, Link-alike is designed specifically for UDP based large file transfer. In their case, the greedy centralized scheduler is sufficient because we just need to have all UDP chunks delivered to the destination without worrying about the order of the chunk arrival and when they arrive.  As we design BaPu, we realize that our design goal of supporting TCP results in some new technical challenges. Due to the TCP's inherent nature, the TCP performance is closely related to whether the TCP sequence can be efficiently delivered in order.  A basic centralized scheduler is no longer adequate to handle TCP transmission.  In section \ref{sec:bapu-pro}, we will propose a new mechanism called \textit{proactive-ACK} to address the challenges of supporting TCP transmission.

\subsection{Load Balancing}

One of our design goals of BaPu is ``fair" sharing of backhaul bandwidth.  In our design, 
``fairness" stands for the following two things,
\begin{itemize}
\item APs are equipped with different uplink bandwidth because they run in different ISP networks, 
and the end users have different subscription plans.  Thus, the BaPu scheduling must be 
``fair" to all the participating BaPu-APs by taking into 
account the available bandwidth of each AP, instead of evenly splitting the traffic among all APs.

\item BaPu is essentially a community based approach by contributing everyone's 
idle bandwidth. We must ensure the ``fairness" to the home LAN users and prioritize
the regular network usage. 
\ignore{The home LAN traffic load may vary depending on how the home LAN users use the network.  }
In order not to disturb the regular network usage, we consistently monitor the ``idle" bandwidth of each BaPu-AP and avoid 
overrunning the uplink. We believe this is critical for such community based approach like BaPu to be 
adopted. 
\end{itemize}

\subsubsection{Why Is FCFS Not Good Enough?}
The FCFS scheduling described in previous section, as suggested by its name, 
is closely related to the latency between BaPu-AP and BaPu-Gateway. 
The BaPu-AP with low latency to the BaPu-Gateway is more likely to be assigned 
with more IP packets because its packet reception report arrives earlier.  
However, the BaPu-AP with low latency might have less uplink bandwidth compared with
other APs. As a result, the FCFS scheduling might place too much traffic load on the APs 
with low latency, and waste a lot of idle bandwidth on other APs with higher latency and
higher bandwidth.  Therefore, FCFS scheduling may result in unfairness among APs.

\subsubsection{Uplink Capacity Estimation}

To avoid this situation, BaPu employs a load balancing mechanism on top of FCFS scheduling.
The core idea of our load balancing mechanism is to combine the estimated available uplink capacity and FCFS 
in scheduling. 

When BaPu-AP sends packet reception report, it piggy back the uplink capacity estimation in the report.  
Since all the IP packets are forwarded through a TCP tunnel connection, therefore the TCP tunnel throughput 
reflects the uplink capacity. We estimate the capacity based on the currently available send buffer size of the 
TCP tunnel socket. The available send buffer size implies how fast the kernel can empty the sender buffer, which 
implies the uplink capacity. BaPu-AP can obtain the available send buffer size by querying the Linux kernel with 
$ioctl()$ function call.  Upon receiving such estimation, BaPu-Gateway decides whether to schedule the IP packets to the 
reporting AP or not. Even though the TCP socket buffer size in the Linux kernel level does not represent the 
exact link capacity, this parameter works very well in our practice, and efficiently balance the load among APs and well adapts to 
the change of capacity. Our capacity estimation matches the method taken in Link-alike \cite{link-alike}.

\input{prelim_exp}


==> diversity.tex <==
\section{Wireless Diversity Gain}



==> evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}
In this section, we conduct a comprehensive set of experiment to evaluate the performance
of BaPu-Pro. First we validate our Proactive-ACK mechanism by comparing 
the TCP throughput of BaPu-Pro against that of BaPu-Basic. Second, we 
measure the performance of BaPu-Pro under a variety of network settings (e.g. network latency, 
background traffic load, wireless link quality, etc.). Finally, we demonstrate that BaPu-Pro is 
feasible for both streaming and large file transfer applications. We conduct 
all the experiments in the same setup as described in section \ref{sec:prelim-exp}.

\subsection{TCP Throughput -- \proack vs. \basic}


\begin{figure*}
\centering
\subfloat[\label{fig:proack_tcp_throughput} \proack vs. -Basic, 32ms RTT, 2Mbps uplink
capacity. ]{\includegraphics[width=\columnwidth]{figures/plot32ms-tcp-compare}\vspace{-0.5cm}}
\subfloat[\label{fig:proack_tcp_th_vs_upper_limit} Efficiency of
Aggregation, BaPu-Basic
vs. BaPu-Pro.]{\includegraphics[width=\columnwidth]{figures/plot32ms-tcp-compare-percent}\vspace{-0.5cm}}
\vspace{-0.2cm}
\caption{TCP aggregated throughput}
\end{figure*}

\ignore{
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/plot32ms-tcp-compare}
\caption{TCP aggregated throughput - \proack vs. \basic, 32ms RTT, 2Mbps uplink capacity. }
\label{fig:proack_tcp_throughput}
\end{figure}

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/plot32ms-tcp-compare-percent}
\caption{Efficiency of Aggregation, BaPu-Basic vs. BaPu-Pro.}
\label{fig:proack_tcp_th_vs_upper_limit}
\end{figure}
}

We carry out the same TCP iperf throughput test as
described in section~\ref{sec:prelim-exp} with BaPu-Pro.  
As shown in Figure~\ref{fig:proack_tcp_throughput}, 
the aggregated TCP throughput of BaPu-Pro significantly outperforms 
that of BaPu-Basic.  With 7 BaPu-APs, BaPu-Pro achieves 11.04Mbps, which
translates to 62\% improvement than BaPu-Basic. Furthermore, Figure~\ref{fig:proack_tcp_th_vs_upper_limit} shows that 
BaPu-Pro achieves at least 88\% aggregation efficiency in our setup, and 
achieves at least 83\% of the upper limit of standard TCP throughput. 

Our experiment results demonstrate that BaPu-Pro can achieve high 
aggregated throughput with high aggregation efficiency for both UDP and TCP.


\subsection{Proactive-ACK Benefit}

To justify our design considerations of Proactive-ACK mechanism, we adopt
the same method as section \ref{sec:bapubasic-tcp} to examine the TCP
CWND growth in BaPu-Basic, BaPu-Pro and normal TCP (Figure 
\ref{fig:tcp_info_basic_vs_proack}).  
In BaPu-Basic, the CWND size remains very small during the whole TCP session. In the contrast, 
BaPu-Pro allows the CWND to grow to very high value, which contributes to the resulting high throughput. 
For reference purpose, we also run a normal TCP session with a throttled bandwidth 11Mbps 
(similar to the BaPu-Pro resulting throughput). The CWND growth patterns for BaPu-Pro and 
normal TCP is very close, which also implies our BaPu-Pro design and implementation can efficiently 
and transparently aggregate multiple slow uplinks.


\begin{figure*}
\centering
\includegraphics[width=2\columnwidth]{figures/plot-basic-7ap-32msrtt-5min-iperf-tcpinfo-cwnd}
\caption{TCP sender CWND growth comparison: \proack vs. \basic vs. normal TCP}
\label{fig:tcp_info_basic_vs_proack}
\end{figure*}
 
\subsection{Impact of Network Latency}
In TCP transmission, the round-trip time (RTT) is an important factor that has impact
on the throughput.  In this experiment, we measure the performance of BaPu-Pro with 4 different network 
latency settings listed in Table \ref{tab:latency}.  Each latency represents certain application scenario. For 
example, when users upload HD video with BaPu to CDN edge servers, the latency to CDN server is generally
regional latency (32ms). When users upload data to their friends in other continent, the RTT is on average 192ms.
Besides, according to our measurement on a residential WiFi testbed, we observe that the latency between broadband
subscribers may vary a lot, ranging between 20ms and 80ms. This depends on whether the two users 
are in the same ISP or different ISPs. Consider the case that a user uploads data with BaPu through 
neighbors' APs to another user in the same city, the latency between the BaPu-APs and the end user can be quite
different. We would like to study the potential impact of the diverse latency on the performance of BaPu-Pro. 
Given certain number of APs, we assign each BaPu-AP a random RTT value between 20ms and 80ms. We carry out 
this test for 10 runs and report the average throughput. As shown in Figure \ref{fig:latency-pro}, BaPu-Pro throughput 
declines as network latency increases, but the throughput reduction is limited. In random latency setting, the 
resulting throughput shows no difference.

\begin{table}
\centering
\caption{\label{tab:latency} Network RTT Latency. Inter-AP RTT
measured by our Open Infrastructure WiFi testbed in Boston area,
representing typical
RTT between home APs in Boston, covering Comcast, RCN, and Verizon.} 
\begin{tabular}{|l|c|}
\hline
Distance & RTT\\
\hline\hline
Regional: 500 - 1,000 mi& 32ms~\cite{akamai:hd}\\
\hline
Cross-continent: $\sim$ 3,000 mi& 96ms~\cite{akamai:hd}\\
\hline
Multi-continent: $\sim$ 6,000 mi& 192ms~\cite{akamai:hd}\\
\hline
inter-AP in Boston& 20ms $\sim$ 80ms\\
\hline
\end{tabular}

\end{table}

%\begin{figure}
%\centering
%\includegraphics[width=\columnwidth]{figures/plot-tcp-latency-compare-7aps}
%\caption{Performance of \basic and \proack for 7 APs with different round-trip time}
%\label{fig:latency-basic-pro-7aps}
%\end{figure}



\begin{figure*}
\centering
\subfloat[\label{fig:latency-pro} Different RTT]{\includegraphics[width=\columnwidth]{figures/plot-proack-tcp-latency-compare}}
\subfloat[\label{fig:diversity-pro} Different packet loss rate $P$ on monitor-APs.]{\includegraphics[width=\columnwidth]{figures/plot-diversity-tcp-compare}}
\caption{BaPu-Pro TCP throughput}
\end{figure*}

\ignore{\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/plot-proack-tcp-latency-compare}
\caption{BaPu-Pro TCP throughput with different RTT}
\label{fig:latency-pro}
\end{figure}
}

\subsection{Impact of Lossy Wireless Links}
%To have a rough idea of the reception performance of overhearing on monitor-APs, 
%we place one sender and one home-AP in the lab, with 5 meter distance.  We placed 
The wireless links in real neighbourhood can be very lossy for a variety 
of reasons, such as cross channel interference and distant neighboring APs. Besides, since monitor-APs 
switch between transmit and receive mode, they cannot overhear all the wireless communication 
happening in the background.
To estimate the potential of BaPu-Pro in a highly lossy wireless environment, we
emulate the packet loss at monitor-APs by dropping the received packets with probability $P$. 
No losses were inflicted on the home-AP, 
because the sender carries out unicast to home-AP, and 802.11 MAC takes care of packet loss
and retransmission. We conduct the experiment with 3 values of $P$, 20\%, 40\% and 60\%. 

As indicated by Figure~\ref{fig:diversity-pro}, the throughput reduction on lossy 
wireless links is very limited in all cases. We believe the good
performance can be explained by the link diversity combined with the
centralized scheduling mechanisms.  The probability of some packet not overheard by 
any monitor-AP is slim, especially when the number of APs is high. This also explains
why 7 BaPu-APs achieve higher throughput with $P=60\%$ than with $P=20\%$. With higher $P$, 
there is still a good chance that some monitor-AP overhears the packet and shares the traffic
load from home-AP. Whereas, less packets are reported to the BaPu-Gateway. The 
reduced control overhead therefore leads to higher effective throughput.

\ignore{
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/plot-diversity-tcp-compare}
\caption{BaPu-Pro TCP throughput with different packet loss rate $P$ on monitor-APs.}
\label{fig:diversity-pro}
\end{figure}
}

%\subsection{Impact of background traffic}
%Figure~\ref{fig:background-traffic}
%
%\begin{figure}
%\centering
%\includegraphics[width=\columnwidth]{figures/plot-proack-bg}
%\caption{Performance of \proack in the presence of background traffic with
%400Kbps uplink and 2.5Mbps download per AP.\label{fig:background-traffic}}
%\end{figure}

\subsection{Streaming vs. Large File Transfer}
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/plot-bursty}
\caption{Instantaneous receiver end throughput. Streaming with 11Mbps transmitter rate vs. iperf }	
\label{fig:bursty}
\end{figure}

During our iperf measurement, even though the average TCP throughput is quite stable in various settings, we find that 
the receiver end instantaneous throughput fluctuates a lot (See Figure \ref{fig:bursty}). 
Our packet trace inspection reveals that due to the latency difference
among APs, the arrival order of the scheduled TCP segments is uncertain. Therefore, the BaPu-Gateway sometimes must buffers 
the out-of-order segments until the expected ones arrive. Besides, since iperf always tries to saturate the link, as the throughput on the WiFi link overruns the aggregated backhual uplink capacity, the out-of-order segment arrival becomes more severe. Both reasons result in the bursty receiver end throughput. 

The iperf throughput only indicates that BaPu is suitable for some applications like instant backup of large files in the cloud. This aligns with the findings of prior work. However, it tells only one side of the story. As we design BaPu, the other important goal is to support instant sharing of high bitrate HD video directly from users' home WiFi, in streaming mode.  The motivation behind such goal is that today's main stream online streaming services (e.g. Netflix) run on TCP based streaming technologies, such as HTTP based Adaptive Bitrate Streaming.  Real time streaming generally requires stable instantaneous throughput.  In this experiment, we would like to study the potential of BaPu as a solution to high bitrate real time streaming. 

Unlike file uploading, streaming application generally has fixed transmitter rate, determined by the codec bit rate. To emulate the streaming traffic, we issue the TCP flow with a tool called \emph{nuttcp}. nuttcp can do rate limiting at transmitter. Figure \ref{fig:bursty} shows the receiver end instantaneous throughput every second in a 100 second session. In the streaming flow with 11Mbps fixed transmitter rate, the receiver end achieves reasonably stable throughput in the whole session. It indicates that BaPu can sustain high bit rate streaming through aggregated links. In comparison, the iperf flow with unlimited transmitter rate shows much higher fluctuation. 

==> prelim_exp.tex <==
\vspace{-0.1in}
\subsection{Preliminary Evaluation}
\label{sec:prelim-exp}
To demonstrate the feasibility and performance of BaPu, we 
first present a preliminary experimental evaluation for BaPu-Basic. 
In this section, we first present our prototype implementation of 
BaPu, and the experiment setup. 
Then, with a set of experimental results, we show that BaPu-Basic achieves 
high aggregation throughput for UDP, but low throughput for TCP.
Our analysis sheds some insight on our design of BaPu-Pro, which significantly 
improves the TCP aggregated throughput. 

\subsubsection{Implementation}
\label{sec:implement}

Both BaPu-AP and BaPu-Gateway are implemented as Linux user space programs
using about 8000 lines of C codes.  Each BaPu-AP has an atheros chipset, running ath9k driver. 
They are configured in both AP mode and monitor mode.
On BaPu-AP, we use \emph{libpcap} to
capture the raw 802.11 traffic from sender.  Since home-AP also forwards the received packets following the
schedules decided by the BaPu-Gateway, we install proper iptables rules to disable the default packet routing through
home-AP. 
We wrote a 802.11 frame
parser and TCP/IP header parser to extract the raw packet information, including
BSSID, IP addresses, ports, etc. 
At BaPu-Gateway, we use
\emph{Linux raw socket} to inject the tunnelled IP packets to the actual 
destination. 
In our prototype, BaPu-AP program is cross-compiled to run on 
commodity home WiFi APs, reflashed with OpenWRT firmware. 
BaPu-Gateway is running on a Linux PC. 


\subsubsection{Experiment Setup}

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/bapu-exp-setup}
\caption{BaPu Experiment Setup. 7 BaPu-APs and 1 BaPu-Gateway are inter-connected. 
Traffic shaping box is setup in between to emulate the typical residential 
network settings. }
\label{fig:bapu-exp-setup}
\end{figure}

Our experiment setup is shown in Figure \ref{fig:bapu-exp-setup}.
Our testbed consists of 1 client, 7 BaPu-APs, 1 BaPu-Gateway, 
1 destination node and a traffic shaping box. Each AP is a Buffalo WZR-HP-G300NH 
802.11n wireless router. This router model has 400MHz CPU and 32MB RAM. 
We have reflashed the APs with OpenWRT firmware, with Linux kernel 2.6.32 
and ath9k WiFi driver. In our experiments, 1 BaPu-AP acts as home-AP which the client 
is always associated to. The other 6 BaPu-APs act as neighbouring monitor-APs to 
capture the traffic in monitor mode. BaPu-Gateway runs on a 
Linux PC, and the destination node runs behind the Gateway 
as an in-LAN node. The legacy client and the destination are both laptops with a 802.11n WiFi card, 
running Ubuntu Linux. 

To emulate the traffic shaping in residential broadband, we install a Linux PC 
between the BaPu-APs and the BaPu-Gateway. We use $tc$ to shape the downlink/uplink bandwidth (htb) to
20Mbps and 2Mbps for downlink and uplink, respectively. 
Also, to emulate the network latency between BaPu-APs and BaPu-Gateway, we use $netem$ tc module to 
shape the latency to 32ms RTT.
The bandwidth and latency parameter is selected by our measurement on our Open Infrastructure urban WiFi testbed,
which represents typical bandwidth capacity and regional latency in the residential cable broadband in Boston urban area. 

In all our experiments, we issue long-lived \emph{iperf} flow
(TCP or UDP) from the client to the destination.  We choose 1350Byte as TCP/UDP 
payload size in our iperf test.  We make sure that the whole client IP packet can be
encapsulated in one IP packet as the BaPu-AP sends it through the TCP tunnel. 
Each iperf test lasts for 30 minutes.
All the throughput value reported in our experiment is the iperf throughput, 
which is the ``goodput". 


\subsubsection{Aggregated Throughput: UDP and TCP}

We evaluate the performance of BaPu-Basic by deploying (up to) 7 BaPu-APs.  
Figure \ref{fig:basic-total-32ms} shows the achieved aggregated throughput with different number of participating APs. 
In UDP, the aggregated throughput increases proportionally with the number of APs. With
7 APs, we achieve 12.4Mbps aggregated UDP throughput. In the contrast, the aggregated TCP throughput does not benefit much when the number of APs increases. The TCP aggregated throughput is always lower than value for UDP in the same setup. With 7 APs, we achieve only 6.83Mbps throughput.


\begin{figure*}
\centering
\subfloat[Throughput for UDP and TCP.  32ms RTT, 2Mbps uplink 
\label{fig:basic-total-32ms}]{\includegraphics[width=\columnwidth]{figures/plot32ms-basic-total}}
\subfloat[\label{fig:basic-total-percent-32ms} Efficiency
for UDP and TCP.  32ms RTT, 2Mbps uplink
]{\includegraphics[width=\columnwidth]{figures/plot32ms-basic-total-percent}}
\caption{BaPu-Basic Aggregation}
\end{figure*}

\ignore{
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/plot32ms-basic-total}
\caption{BaPu-Basic Aggregated Throughput for UDP and TCP.  32ms RTT, 2Mbps uplink}
\label{fig:basic-total-32ms}
\end{figure}
}

\subsubsection{Aggregation Efficiency}

Asides from the aggregated throughput, we use another metric, \emph{Aggregation Efficiency}, to evaluate the performance of BaPu.  We define the Aggregation Efficiency as the ratio of the resulting throughput over the maximum theoretical goodput.  Due to the TCP/IP header and BaPu protocol overhead, the actual goodput is less than the uplink capacity.  With all protocol header overhead accounted, we derive the maximum theoretical goodput given backhaul capacity of 2Mbps.  
Table \ref{tab:limit} lists the maximum throughput when data is transmitted via UDP/TCP standard protocol and via our BaPu system. 

\begin{table}
\centering
\begin{tabular}{|l|c|}
\hline
Uplink Capacity & 2 Mbps\\
\hline \hline
max UDP & 1.94 Mbps\\
\hline
max \mytit UDP & 1.82 Mbps\\
\hline
max TCP & 1.9 Mbps\\
\hline
max \mytit TCP & 1.8 Mbps\\
\hline
\end{tabular}
\caption{Maximum theoretical goodput for TCP and UDP. Data payload size is 1350Byte.}
\label{tab:limit}
\end{table}

As shown in Figure~\ref{fig:basic-total-percent-32ms}, BaPu-Basic UDP can harness close to 100\% idle
bandwidth. Even if we consider the extra overhead incurred by BaPu protocol messages, UDP aggregation 
efficiency is still over 90\% in all cases.  In the contrast, the aggregation efficiency for TCP degrades 
quickly as more APs join the cooperation. With 7 BaPu-APs, we transform only 50\% of idle bandwidth 
to effective throughput. 

This shows that 1) our BaPu-Basic mechanism design is efficient for UDP; 2)
our prototype implementation is efficient from engineering perspective.  
Next, we discuss the reasons for poor TCP performance in BaPu-Basic.

\ignore{
\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/plot32ms-basic-total-percent}
\caption{BaPu-Basic Efficiency of Aggregation for UDP and TCP.  32ms RTT, 2Mbps Uplink Capacity}
\label{fig:basic-total-percent-32ms}
\end{figure}
}
\subsubsection{A Look inside Poor TCP Performance}
\label{sec:bapubasic-tcp}
In this section we carry out an in-depth analysis on TCP behaviour in BaPu-Basic. 
Our analysis reveals that some TCP inherent nature 
raises some challenges, and limits the throughput with 
the simple design of BaPu-Basic.

TCP ensures successful and in-order data delivery between the 
sender and the receiver. 
\ignore{TCP relies on two major mechanisms, flow control and congestion control. 
The former one prevents the sender from overrunning the receiver buffer. The latter one prevents the sender from overrunning the network path between the sender and the receiver.}
 In TCP, each packet is 
identified with a sequence number and must be acknowledged by the receiver 
to indicate the proper delivery. The sender maintains a dynamic CWND (Congestion Window) 
as the communication goes on, which indicates the maximum number of packets on 
the fly. If some packet is not ACK'ed before RTO (Retransmission Timeout) occurs, 
the sender issues retransmission. If the receiver receives some out-of-order sequence, this generally implies that the missing sequence number is lost or delayed due 
to congested network. In this case, the receiver sends a DUPACK (Duplicate ACK) 
to inform the sender of the missing sequence. By default, the sender issues 
Fast\_Retransmission upon receiving 3 DUPACKs. In either of these two cases, the sender 
reduces the CWND accordingly to slow down the sending rate and adapt to the congested 
network or slow receiver. 

TCP was designed based on the fact that the out-of-order 
sequence is generally a good indicator of packet being lost or the network path is 
experiencing congestion. However, such assumption no longer holds 
in BaPu. In BaPu, the packets belonging to the same TCP session are intentionally routed through 
multiple APs, which have diverse backhaul connections in terms of capacity, 
latency, traffic load, etc. This results in very serious out-of-order packet at 
the BaPu-Gateway. As BaPu-Gateway forwards the out-of-order packets to the
destination, the sender and destination falls on the TCP congestion control mechanism to limit the 
CWND at a very low value. The throughput is consequently highly limited.

To further justify our analysis, we inspect the TCP behaviour by examining
the Linux kernel TCP stack variables. We use the $getsockopt()$
call to query the $TCP\_INFO$ Linux kernel data structure. 
$TCP\_INFO$ includes system time stamp, sender
CWND, retransmissions, etc.  We have modified the iperf client to log 
$TCP\_INFO$ each time when 
iperf calls send() to write the application buffer data to the TCP 
socket buffer.  
Figure \ref{fig:plot-basic-7ap-32msrtt-5min-iperf-tcpinfo-cwnd-retrans}
shows how TCP CWND grows in a 120 second iperf test with 7 BaPu-APs. 
With 7 APs, we expect to obtain $2Mbps\times7 = 14Mbps$ throughput.
In comparison, we carry out another iperf test with normal TCP through a 
regular AP with 14Mbps uplink capacity.  The CWND growth in normal TCP 
connection is also shown in Figure \ref{fig:plot-basic-7ap-32msrtt-5min-iperf-tcpinfo-cwnd-retrans}.
In BaPu-Basic TCP session, the sender side congestion window remains
at a very low level.  Our pcap captured packet trace at client shows that a lot 
of DUPACKs and RTO timeout incurs a lot of retransmissions, which results in 
very low TCP throughput. 

\begin{figure}
\centering
\includegraphics[width=\columnwidth]{figures/plot-basic-7ap-32msrtt-5min-iperf-tcpinfo-cwnd-retrans}
\caption{TCP sender CWND growth, BaPu-Basic vs. normal TCP. 32ms RTT and 2Mbps uplink }
\label{fig:plot-basic-7ap-32msrtt-5min-iperf-tcpinfo-cwnd-retrans}
\end{figure}


==> setup.tex <==
\section{Problem Statement and \\Architectural Challenges}


 shows our system setup. In a residential area, a
client device, the ``source'' $S$, sends large amounts of data
wirelessly to a destination $D$. As an example scenario, imagine a
user with a handheld device wirelessly uploading a large video to
YouTube.  Therefore, client $S$ connects to its home access point
$\hap{H}$ which is connected to the Internet and forwards data to
$D$. However, it turns out that the performance problem in this
scenario is the throttled backhaul of $\hap{H}$.  Typically, the
wireless channel between $S$ and $\hap{H}$ offers a higher throughput
than $\hap{H}$'s Internet backhaul.  For example, 802.11n provides
$T_{\mathrm{Wifi}}=54$ Mbps to $T_{\mathrm{Wifi}}=600$ Mbps while,
today, typical cable backhauls are throttled by Internet providers to
a throughput between $T_\mathrm{backhaul}= 1$ Mbps and
$T_\mathrm{backhaul}= 3$ Mbps.

Yet, in residential areas, there is often more than just the home
access point $\hap{H}$ in communication range to $S$ (typically tens of APs). That is, a list
of $n$ access points $\{\hap{1},\ldots{},\hap{n}\}$ can overhear (some
of the) packets sent from $S$ to $\hap{H}$. If these ``neighboring''
access points are idle, it seems straightforward to utilize their
spare backhaul capacity and assist $S$ in delivering its data more
quickly to $D$. The main rationale is to \emph{split} the burden of
delivering $S$'s packets among all APs in communication range. 
However, such a system faces several challenges.

\paragraph{Challenges}
\vskip 2eX \noindent{\bf Client Transparency:} First of all, for
client $S$, the system should work transparently. There should be no
requirement to change $S$'s network stack. For $S$, the system should
look like standard, e.g., TCP communication with $D$. This is
motivated by the enormous heterogeneity of possible end user
devices. Changing details of the network stack would need to be
implemented and maintained on many different architectures. Instead,
for the massive deployment of such a system, we argue that only the
APs' and destination $D$'s network stack should undergo changes. For
the real-world, we expect this to be much more feasible. For example,
Internet service providers and AP manufacturers can cooperate with
content providers such as YouTube.
  

\vskip 1eX\noindent{\bf Lightweight Coordination:} As backhauls
represent a major bottleneck for throughput, the system must refrain
as much as possible from inter-AP coordination. If APs communicate
with each other to, e.g., schedule packet delivery towards $S$, this
puts additional load on backhauls degrading the overall throughput. 


\vskip 1eX\noindent{\bf TCP and Packet Loss:} The scenario requires
reliable end-to-end data delivery. Although not primarily designed for
wireless environments, TCP has to be employed for the communication
from $S$ to $D$. This will keep client transparency and allow system
usage with legacy protocols.  Communication between APs and $D$ traverses
the Internet and has to be
``TCP-friendly''~\cite{tcp-friendly,tcp-friendly2}.  \ignore{While UDP-based
systems can be envisioned that emulate congestion control mechanisms,
TCP must also be used for Internet communication between the $\hap{i}$
and $D$.}

Yet, with TCP-based communication, packet loss in our wireless
environment has a severe impact on throughput.  Packet loss results in
either a time-out or out of order TCP delivery. This causes the TCP
window size to be cut in half.  While the \emph{primary} wireless link
between $S$ and $\hap{H}$ employs ARQ for reliable packet delivery at
$\hap{H}$, the \emph{secondary} wireless link to neighbors $\hap{i}$
is prone to packet loss.  Due to the space diversity of the APs, the
packet loss at each AP is different.  Consequently, besides $\hap{H}$,
neighboring APs receive different subsets of sent packets. As AP
should not exchange information, it is difficult to coordinate which
AP has received which packet.  A system has to take this into account.

\vskip 1eX\noindent{\bf Out-of-Order Packets:} All APs use standard
TCP communication with $S$.  Consequently, packet loss is not the only
reason for out-of-order packet receipt at $S$, but the difference in
latencies between APs and $S$ is another one. A low latency AP can
deliver its packets before a high latency AP. At receiver $D$, TCP
packets will arrive with out of order sequence numbers.  Assuming
dropped packets, $D$ typically responses with duplicate
acknowledgments (``DUPACK''), requesting the client to reduce its
sending rate. After $S$ has received 3 DUPACKs, it will start a fast
retransmit hurting overall throughput.

In our scenario however, out-of-order packets are main\-ly caused by
backhaul latency differences among APs and, generally, the multipath
setup with different arrival characteristics.  The system needs to
avoid generating duplicate ACKs (and dividing TCP's window size in
half).


\vskip 1eX\noindent{\bf Embedded Devices:} While many complex systems
for bunching neighboring access points can be envisioned, we have to
take the extreme resource restrictions of cheap, commodity hardware
APs into account. APs are powered with embedded hardware,
featuring only a few MBs of main memory and comparably lightweight
CPUs. Typically, already forwarding of packets between the
wireless interface to the backhaul uses an AP's CPU to full
capacity. Consequently, the system restrains to simple operations, as
complex operations would overburden APs.

We will now present the design of \mytit and explain how \mytit
addressed the individual research challenges.

